Technical Design Report for the: PANDA Micro Vertex Detector

This document illustrates the technical layout and the expected performance of the Micro Vertex Detector (MVD) of the PANDA experiment. The MVD will detect charged particles as close as possible to the interaction zone. Design criteria and the optimisation process as well as the technical solutions chosen are discussed and the results of this process are subjected to extensive Monte Carlo physics studies. The route towards realisation of the detector is outlined.

==> sty/panda_commands.tex <==
% def_panda_cmd.tex
%
\RequirePackage[centertags]{amsmath}
%
\RequirePackage{xspace}
%\RequirePackage{ulem}
%
%\def\MARK#1{\texorpdfstring{{\emph{\textcolor{red}{#1}}}}{{#1}}}
%\def\MARK#1{\emph{\textcolor{red}{#1}}}
%\def\MARK#1{{\bf \textcolor{red}{#1}}}
%\def\MARK#1{{#1}}
% use to mark text 
% (Text will be kept, but the marking removed in the final document)
%
\def\COM#1{\fbox{\parbox{\swidth}{\textcolor{red}{\bf COMMENT: #1}}}}
%\def\COM#1{}
% use to add comments
% (The whole will be removed in the final version)
%
% use to mark parts, which shouldn't be present in the cost-free version

\def\OnlyLayoutColumnBreak{{\vfill\newpage}}%

\def\OnlyLayoutPageBreak{{\vfill\clearpage}}%

\def\OnlyLayoutDoublePageBreak{{\vfill\cleardoublepage}}%

%
\def\bfg{\begin{figure}}%
\def\efg{\end{figure}}%
\def\bc{\begin{center}}%
\def\ec{\end{center}}%
\def\bi{\begin{itemize}}%
\def\ei{\end{itemize}}%
\def\beq{\begin{equation}}%
\def\eeq{\end{equation}}%
\def\bn{\begin{eqnarray}}%
\def\en{\end{eqnarray}}%
\def\ba#1{\left(\begin{array}{#1}}%
\def\ea{\end{array}\right)}%
\def\bef{\begin{equation}\fbox{$\displaystyle}%
\def\eef{$}\end{equation}}%
\def\bnf{\bef\ba{rcl}}%
\def\enf{\ea\eef}%
\newcommand{\beal}{\begin{align}}
\newcommand{\eal}{\end{align}}
\newcommand{\bespl}{\begin{split}}
\newcommand{\espl}{\end{split}}
%\def\refeq#1{\Eqref{#1}\xspace}%
%\def\Refsec#1{sec.~\ref{#1}\xspace}%
%\def\Refchap#1{\Refchap{#1}\xspace}%
%\def\Reffig#1{\Reffig{#1}\xspace}%
%\def\Reftbl#1{\Reftbl{#1}\xspace}%
%\def\reftab#1{\Reftbl{#1}\xspace}%
\def\Refeq#1{Eq.~\ref{#1}\xspace}%
\def\Refeqs#1{Eqs.~\ref{#1}\xspace}%
\def\Refsec#1{Sec.~\ref{#1}\xspace}%
\def\Refchap#1{Chap.~\ref{#1}\xspace}%
\def\Reffig#1{Fig.~\ref{#1}\xspace}%
\def\Reffigs#1{Figs.~\ref{#1}\xspace}%
\def\Reftbl#1{Table~\ref{#1}\xspace}%
\def\Reftbls#1{Tables~\ref{#1}\xspace}%
\def\RefeqX#1{Eq.~\ref{#1}}%
\def\RefeqsX#1{Eqs.~\ref{#1}}%
\def\RefsecX#1{Sec.~\ref{#1}}%
\def\RefchapX#1{Chap.~\ref{#1}}%
\def\ReffigX#1{Fig.~\ref{#1}}%
\def\ReffigsX#1{Figs.~\ref{#1}}%
\def\ReftblX#1{Table~\ref{#1}}%
\def\ReftblsX#1{Tables~\ref{#1}}%
%\def\Reftab#1{Table~\ref{#1}\xspace}%
\def\ub{\underbrace}%
%
\def\vps{\hspace*{5mm}}%
\def\dsty{\displaystyle}%
%
\newcounter{auth}%
\setcounter{auth}{0}%
\def\authitem#1{\addtocounter{auth}{1}#1}%
\def\authitemi#1#2{\addtocounter{auth}{1}#2$^{#1}$}%
\newcounter{inst}%
\setcounter{inst}{0}%
\def\institem#1{\par \addtocounter{inst}{1}#1\\}%
\def\lastitem{\ }%
\def\respitem#1{\institem{{\bf #1}\lastitem\\}}%
\let\groupitem=\authitem
%
\newcommand{\captionfonts}{\small}
%
\makeatletter  % Allow the use of @ in command names
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts {\bf #1:} #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts {\bf #1:} #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother   % Cancel the effect of \makeatletter
%
% a few commands to change the figure placing (commented are the default values)
%\renewcommand{\textfraction}{0.1} % 0.2
%\renewcommand{\bottomfraction}{0.4} % 0.3
%\renewcommand{\dbltopfraction}{0.8} % 0.7
%\renewcommand{\dblfloatpagefraction}{0.3} % 0.5
%\renewcommand{\floatpagefraction}{0.3} % 0.5
%\setcounter{dbltopnumber}{3} % 2
%\setcounter{bottomnumber}{2} % 1
%
%\def\markpanda#1#2{\markboth{\Panda{} - #1}{FAIR/Pbar/#2}}%
\def\markpanda#1#2{\markboth{\Panda{} - #1}{FAIR/PANDA/#2}}%
%
\newcommand{\unit}[1]{\,\mathrm{#1}}

% EOF: def_panda_cmd.tex


==> sty/panda_detector.tex <==
% panda_detector.tex
%
\RequirePackage{xspace}
%
\def\INST#1{\texorpdfstring{{\sffamily #1}}{{#1}}\xspace}%
%
\def\PANDA{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\Panda{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\panda{\texorpdfstring{$\overline{\mbox{\sffamily P}}${\sffamily ANDA}}{Panda}\xspace}%
\def\HESR{\INST{HESR}}%
\def\Hesr{\INST{HESR}}%
\def\GSI{\INST{GSI}}%
\def\Gsi{\INST{GSI}}%
\def\FAIR{\INST{FAIR}}%
\def\Fair{\INST{FAIR}}%
%
% General definitions
%
\def\Ts{TS\xspace}
\def\Fs{FS\xspace}
\def\Mvd{MVD\xspace}
\def\Emc{EMC\xspace}
\def\TsEmc{TS-EMC\xspace}
\def\FsEmc{FS-EMC\xspace}
\def\Had{HAD\xspace}
\def\Muo{MUO\xspace}
\def\TsMuo{TS-MUO\xspace}
\def\FsMuo{FS-MUO\xspace}
\def\Stt{STT\xspace}
\def\Tpc{TPC\xspace}
\def\Dirc{DIRC\xspace}
\def\Rich{RICH\xspace}
\def\Mdc{MDC\xspace}
\def\TsMdc{TS-MDC\xspace}
\def\FsMdc{FS-MDC\xspace}
\def\Tof{TOF\xspace}
\def\Lum{LUM\xspace}
\def\Mag{MAG\xspace}
\def\TsMag{SOL\xspace}
\def\FsMag{DIP\xspace}

\def\frontend{front-end\xspace}
\def\frontends{front-ends\xspace}
\def\Frontend{Front-end\xspace}
\def\Frontends{Front-ends\xspace}
%\def\fe{front-end }

%
% EMC definitions
%
\def\BEMC{barrel EMC\xspace}
\def\FWEMC{forward endcap EMC\xspace}
\def\BWEMC{backward endcap EMC\xspace}
\def\TSEMC{target spectrometer EMC\xspace}
\def\FSEMC{forward spectrometer EMC\xspace}
\def\TsEmc{\TSEMC}
\def\FsEmc{\FSEMC}
%
\def\LAAPD{LAAPD\xspace}
\def\LAAPDs{LAAPDs\xspace}
\def\VPT{VPT\xspace}
\def\VPTs{VPTs\xspace}
\def\PWOII{PWO-II\xspace}
\def\PWO{PWO\xspace}

% EOF: def_panda_det.tex


==> sty/panda_symbols.tex <==
% def_panda_sym.tex
%
\input{sty/pennames.sty}
\input{sty/myunits.sty}
\input{sty/mymath.sty}
%
\RequirePackage{xspace}
% Upright mu for micro
\DeclareFontFamily{U}{euc}{}% I chose euc because the chart is called Euler cursive
\DeclareFontShape{U}{euc}{m}{n}{<-6>eurm5<6-8>eurm7<8->eurm10}{}%
\DeclareSymbolFont{AMSc}{U}{euc}{m}{n} % I chose AMSc because AMSa and AMSb are defined in the amsfonts-package
\DeclareMathSymbol{\umu}{\mathord}{AMSc}{"16}
%
\def\degrees{\ensuremath{^\circ}\xspace}%
\def\percent{$\,$\%\xspace}%
\def\prm{\ensuremath{^\prime}}%
\def\etc{{\em etc.}\xspace}%
%
% theory stuff
%
\newcommand{\MZ}{M^{\!\!\!\!\!^o}}
\newcommand{\aslash}{\FMslash a}
\newcommand{\Partialslash}{\FMslash \partial}
\newcommand{\vslash}{\FMslash v}
\newcommand{\pslash}{\FMslash p}
\newcommand{\wslash}{\FMslash w}
\newcommand{\lslash}{\FMslash l}
\newcommand{\Lslash}{\FMslash L}
\newcommand{\qslash}{\FMslash q}
\newcommand{\Qslash}{\FMslash Q}
\newcommand{\Pslash}{\FMslash P}
\newcommand{\Wslash}{\FMslash W}
\newcommand{\kslash}{\FMslash k}
\newcommand{\Kslash}{\FMslash K}
\newcommand{\barKslash}{\FMslash {\bar K}}
\newcommand{\barPslash}{\FMslash {\bar P}}
\newcommand{\kapslash }{\FMslash \kappa }
\newcommand{\chiral}[1]{\stackrel{\circ}{#1}}
\def\Re{{\rm Re\,}}
\def\Im{{\rm Im\,}}
\def\prt{\partial}
%
\def\BW{\ensuremath{\mbox{\it BW}}\xspace}%
\def\BR{\ensuremath{\mathcal{B}}\xspace}%
\def\LH{\ensuremath{\mathcal{L}}\xspace}%
\def\CL{\ensuremath{\mbox{\it CL}}\xspace}%
%
\def\vloo{\mbox{\tt VeryLoose}\xspace}
\def\loo{\mbox{\tt Loose}\xspace}
\def\tig{\mbox{\tt Tight}\xspace}
\def\vtig{\mbox{\tt Tight}\xspace}
%
\def\tm{\texttrademark}
\def\tmr{\ensuremath{^{\textregistered}}}
%
%\def\ppbar{\ensuremath{\mbox{p}\overline{\mbox{p}}}\xspace}% non-italic
\def\ppbar{\ensuremath{p\overline{p}}\xspace}% italic
%\def\pbarp{\ensuremath{\overline{\mbox{p}}\mbox{p}}\xspace}% non-italic
\def\pbarp{\ensuremath{\overline{p}p}\xspace}% italic
\def\NNbar{\ensuremath{N\overline{N}}\xspace}% italic
%\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}% non-italic
\def\pbard{\ensuremath{\overline{p}d}\xspace}% italic
%\def\pbarA{\ensuremath{\overline{\mbox{p}}\mbox{A}}\xspace}% non-italic
\def\pbarA{\ensuremath{\overline{p}A}\xspace}% italic
%\def\pbarAu{\ensuremath{\overline{\mbox{p}}\mbox{Au}}\xspace}% non-italic
\def\pbarAu{\ensuremath{\overline{p}Au}\xspace}% italic
%\def\pbarN{\ensuremath{\overline{\mbox{p}}\mbox{N}}\xspace}% non-italic
\def\pbarN{\ensuremath{\overline{p}N}\xspace}% italic
%\def\pbar{\ensuremath{\overline{\mbox{p}}}\xspace}%s non-italic
\def\pbar{\ensuremath{\overline{p}}\xspace}%s italic
%\def\nbar{\ensuremath{\overline{\mbox{n}}}\xspace}% non-italic
\def\nbar{\ensuremath{\overline{n}}\xspace}% italic
%\def\pbarn{\ensuremath{\overline{\mbox{p}}\mbox{n}}\xspace}% non-italic
\def\pbarn{\ensuremath{\overline{p}n}\xspace}% italic
%\def\nbarn{\ensuremath{\overline{\mbox{n}}\mbox{n}}\xspace}% non-italic
\def\nbarn{\ensuremath{\overline{n}n}\xspace}% italic
\def\NbarN{\ensuremath{\overline{N}N}\xspace}% italic
%
\def\qbar{\ensuremath{\overline{q}}\xspace}% italic
\def\cbar{\ensuremath{\overline{c}}\xspace}% italic
\def\ccbar{\ensuremath{c\overline{c}}\xspace}% italic
\def\ccbarg{\ensuremath{c\overline{c}g}\xspace}% italic
\def\cqbar{\ensuremath{c\overline{q}}\xspace}% italic
\def\cbarq{\ensuremath{\overline{c}q}\xspace}% italic
\def\uubar{\ensuremath{u\overline{u}}\xspace}% italic
\def\ddbar{\ensuremath{d\overline{d}}\xspace}% italic
\def\ssbar{\ensuremath{s\overline{s}}\xspace}% italic
\def\bbbar{\ensuremath{b\overline{b}}\xspace}% italic
\def\bqbar{\ensuremath{b\overline{q}}\xspace}% italic
\def\bbarq{\ensuremath{\overline{b}q}\xspace}% italic
\def\qqbar{\ensuremath{q\overline{q}}\xspace}% italic
\def\qqbarg{\ensuremath{q\overline{q}g}\xspace}% italic
\def\QQbar{\ensuremath{Q\overline{Q}}\xspace}% italic
%
\def\ee{\ensuremath{e^+e^-}\xspace}%
\def\mumu{\ensuremath{\mu^+\mu^-}\xspace}%
%
\def\piz{\ensuremath{\pi^0}\xspace}%
\def\pip{\ensuremath{\pi^+}\xspace}%
\def\pim{\ensuremath{\pi^-}\xspace}%
\def\pipm{\ensuremath{\pi^\pm}\xspace}%
\def\pimp{\ensuremath{\pi^\mp}\xspace}%
%
\def\K{\ensuremath{K}\xspace}%
\def\Kp{\ensuremath{K^+}\xspace}%
\def\Km{\ensuremath{K^-}\xspace}%
\def\Kpm{\ensuremath{K^\pm}\xspace}%
\def\Kmp{\ensuremath{K^\mp}\xspace}%
\def\KKbar{\ensuremath{K\overline{K}}\xspace}%
\def\Kz{\ensuremath{K^0}\xspace}%
\def\Kbar{\ensuremath{\overline{K}}\xspace}%
\def\Kzbar{\ensuremath{\overline{K}^0}\xspace}%
\def\KzKzbar{\ensuremath{K^0\overline{K^0}}\xspace}%
\def\Ks{\ensuremath{K_S^0}\xspace}%
\def\Kl{\ensuremath{K_L^0}\xspace}%
%
\def\etaprime{\ensuremath{\eta\prm}\xspace}%
\def\pione{\ensuremath{\pi_1}\xspace}%
%
\def\uquark{\ensuremath{u}\xspace}%
\def\dquark{\ensuremath{d}\xspace}%
\def\squark{\ensuremath{s}\xspace}%
\def\cquark{\ensuremath{c}\xspace}%
\def\bquark{\ensuremath{b}\xspace}%
\def\tquark{\ensuremath{t}\xspace}%
%
\def\D{\ensuremath{D}\xspace}%
\def\Dbar{\ensuremath{\overline{D}}\xspace}%
\def\DDbar{\ensuremath{D\overline{D}}\xspace}%
\def\DpDm{\ensuremath{D^+D^-}\xspace}%
\def\Dp{\ensuremath{D^+}\xspace}%
\def\Dm{\ensuremath{D^-}\xspace}%
\def\Dz{\ensuremath{D^0}\xspace}%
\def\Dzbar{\ensuremath{\overline{D}^0}\xspace}%
\def\DzDzbar{\ensuremath{D^0\overline{D}^0}\xspace}%
\def\DzDzxbar{\ensuremath{D^0\overline{D}^{\ast0}}\xspace}%
\def\Dx{\ensuremath{D^\ast}\xspace}%
\def\Dxbar{\ensuremath{\overline{D}^\ast}\xspace}%
\def\DxDxbar{\ensuremath{D^\ast\overline{D}^\ast}\xspace}%
\def\Dxz{\ensuremath{D^{\ast 0}}\xspace}%
\def\Dxzbar{\ensuremath{\overline{D}^{\ast 0}}\xspace}%
\def\DbarDxx{\ensuremath{D\overline{D}^{\ast\ast}}\xspace}%
%
\def\Ds{\ensuremath{D_s}\xspace}%
\def\Dspm{\ensuremath{D_s^\pm}\xspace}%
\def\Dsmp{\ensuremath{D_s^\mp}\xspace}%
\def\Dsx{\ensuremath{D_s^\ast}\xspace}%
\def\Dsxpm{\ensuremath{D_s^{\ast\pm}}\xspace}%
\def\Dsxmp{\ensuremath{D_s^{\ast\mp}}\xspace}%
\def\DsDsbar{\ensuremath{D_s\overline{D_s}}\xspace}%
\def\DspDsm{\ensuremath{D_s^+D_s^-}\xspace}%
\def\DsxDsxbar{\ensuremath{D_s^\ast\overline{D_s}^\ast}\xspace}%
\def\DsbarDsxx{\ensuremath{\overline{D_s}D_s^{\ast\ast}}\xspace}%
%
\def\jpsi{\ensuremath{J\!/\!\psi}\xspace}%
\def\psiprime{\ensuremath{\psi\prm}\xspace}%
\def\etac{\ensuremath{\eta_c}\xspace}%
\def\etacprime{\ensuremath{\eta\prm_c}\xspace}%
\def\chicJ{\ensuremath{\chi_{cJ}}\xspace}%
\def\chiczero{\ensuremath{\chi_{c0}}\xspace}%
\def\chicone{\ensuremath{\chi_{c1}}\xspace}%
\def\chictwo{{\chi_{c2}}\xspace}%
\def\honec{\ensuremath{h_c}\xspace}%
%
\def\Lambdaplain{\ensuremath{\varLambda}\xspace}% italic
\def\Lambdabar{\ensuremath{\overline{\varLambda}}\xspace}%
\def\LambdaLambdabar{\ensuremath{\varLambda\overline{\varLambda}}\xspace}%
\def\Omegaplain{\ensuremath{\varOmega}\xspace}% 
\def\Omegabar{\ensuremath{\overline{\varOmega}}\xspace}%
\def\OmegaOmegabar{\ensuremath{\varOmega\overline{\varOmega}}\xspace}%
\def\Sigmabar{\ensuremath{\overline{\varSigma}}\xspace}%
\def\Sigmaplain{\ensuremath{\varSigma}\xspace}%
\def\SigmaSigmabar{\ensuremath{\varSigma\overline{\varSigma}}\xspace}%
\def\Cascade{\ensuremath{\varXi}\xspace}%
\def\Cascadebar{\ensuremath{\overline{\varXi}}\xspace}%
\def\Cascademinus{\ensuremath{\varXi^-}\xspace}% 
\def\CascadeCascadebar{\ensuremath{\varXi\overline{\varXi}}\xspace}% 
\def\Lambdac{\ensuremath{\varLambda_c}\xspace}%
\def\Sigmac{\ensuremath{\varSigma_c}\xspace}%
\def\Omegac{\ensuremath{\\varOmega_c}\xspace}%
\def\Cascadec{\ensuremath{\varXi_c}\xspace}%
%
\def\kev{{\mbox{keV}}\xspace}%
\def\kevcc{{\mbox{keV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mev{{\mbox{MeV}}\xspace}%
\def\mevc{{\mbox{MeV}\!/\!\mbox{\em c}}\xspace}%
\def\mevcc{{\mbox{MeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mevccsq{{\mbox{MeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
\def\gev{{\mbox{GeV}}\xspace}%
\def\gevc{{\mbox{GeV}\!/\!\mbox{\em c}}\xspace}%
\def\gevcsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevcc{{\mbox{GeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevccsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
\def\neueq{$\mathrm{ n_{1 MeV\,eq}\,cm^{-2}}$\xspace}%
%
\def\aC{{\mbox{aC}}\xspace}%
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\mubarn{\ensuremath{\rm \,\mu b}\xspace}
\def\nb{\ensuremath{\rm \,nb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
%
\def\JPC{\ensuremath{J^{\!P\!C}}\xspace}%
\def\JPCzeropm{\ensuremath{0^{+-}}\xspace}%
\def\JPCzeropp{\ensuremath{0^{++}}\xspace}%
\def\JPCzeromm{\ensuremath{0^{--}}\xspace}%
\def\JPCzeromp{\ensuremath{0^{-+}}\xspace}%
\def\JPConepm{\ensuremath{1^{+-}}\xspace}%
\def\JPConepp{\ensuremath{1^{++}}\xspace}%
\def\JPConemm{\ensuremath{1^{--}}\xspace}%
\def\JPConemp{\ensuremath{1^{-+}}\xspace}%
\def\JPCtwopm{\ensuremath{2^{+-}}\xspace}%
\def\JPCtwopp{\ensuremath{2^{++}}\xspace}%
\def\JPCtwomm{\ensuremath{2^{--}}\xspace}%
\def\JPCtwomp{\ensuremath{2^{-+}}\xspace}%
%
\def\JPCscalar{\JPCzeropp}%
\def\JPCvector{\JPConemm}%
\def\JPCtensor{\JPCtwopp}%
%
\def\GE {\relax\ifmmode{\rm G_E}%
         \else${\rm G_E}$\fi}
\def\GM {\relax\ifmmode{\rm G_M}%
         \else${\rm G_M}$\fi}
\def\Fi {\relax\ifmmode{\rm F_1}%
         \else${\rm F_1}$\fi}
\def\Fii {\relax\ifmmode{\rm F_2}%
         \else${\rm F_1}$\fi}
\def\qsq {\relax\ifmmode{\rm q^2}%
         \else${\rm q^2}$\fi}
%
\def\tO{\,\rightarrow\,}
%
\def\extl{\ensuremath{E_{xtl}}\xspace}
\def\ecl{\ensuremath{E_{cl}}\xspace}
\def\emax{\ensuremath{E_{max}}\xspace}
%
% EOF: def_panda_sym.tex

